Frobenius lifts and elliptic curves with complex multiplication

We give a new characterisation of elliptic curves of Shimura type in terms commuting families of Frobenius lifts and also strengthen an old principal ideal theorem for ray class fields. These two results combined yield the existence of global minimal models for elliptic curves of Shimura type, generalising a result of Gross. Along the way we also prove a handful of small but new results regarding elliptic curves with complex multiplication.

==> custom.tex <==
%UPSHAPE LETTERS IN MATH MODE
\typeout{Style Option: `Upshape Caps letters in math mode'}
\DeclareMathSymbol{A}{\mathalpha}{operators}{`A}%
\DeclareMathSymbol{B}{\mathalpha}{operators}{`B}%
\DeclareMathSymbol{C}{\mathalpha}{operators}{`C}%
\DeclareMathSymbol{D}{\mathalpha}{operators}{`D}%
\DeclareMathSymbol{E}{\mathalpha}{operators}{`E}%
\DeclareMathSymbol{F}{\mathalpha}{operators}{`F}%
\DeclareMathSymbol{G}{\mathalpha}{operators}{`G}%
\DeclareMathSymbol{H}{\mathalpha}{operators}{`H}%
\DeclareMathSymbol{I}{\mathalpha}{operators}{`I}%
\DeclareMathSymbol{J}{\mathalpha}{operators}{`J}%
\DeclareMathSymbol{K}{\mathalpha}{operators}{`K}%
\DeclareMathSymbol{L}{\mathalpha}{operators}{`L}%
\DeclareMathSymbol{M}{\mathalpha}{operators}{`M}%
\DeclareMathSymbol{N}{\mathalpha}{operators}{`N}%
\DeclareMathSymbol{O}{\mathalpha}{operators}{`O}%
\DeclareMathSymbol{P}{\mathalpha}{operators}{`P}%
\DeclareMathSymbol{Q}{\mathalpha}{operators}{`Q}%
\DeclareMathSymbol{R}{\mathalpha}{operators}{`R}%
\DeclareMathSymbol{S}{\mathalpha}{operators}{`S}%
\DeclareMathSymbol{T}{\mathalpha}{operators}{`T}%
\DeclareMathSymbol{U}{\mathalpha}{operators}{`U}%
\DeclareMathSymbol{V}{\mathalpha}{operators}{`V}%
\DeclareMathSymbol{W}{\mathalpha}{operators}{`W}%
\DeclareMathSymbol{X}{\mathalpha}{operators}{`X}%
\DeclareMathSymbol{Y}{\mathalpha}{operators}{`Y}%
\DeclareMathSymbol{Z}{\mathalpha}{operators}{`Z}%

%CATEGORIES NOTATIONS
\newcommand{\coker}{\mathrm{coker}}
\newcommand{\im}{\mathrm{im}}
\newcommand{\isomto}{\overset{\sim}{\longrightarrow}}
\newcommand{\mto}{\mapsto}
\DeclareMathOperator*{\colim}{colim}

%CATEGORIES
\newcommand{\Aff}{\mathrm{Aff}}
\newcommand{\IndAff}{\mathrm{IndAff}}
\newcommand{\IndSch}{\mathrm{IndSch}}
\newcommand{\QCoh}{\mathrm{QCoh}}
\newcommand{\Cat}{\mathrm{Cat}}
\newcommand{\Fib}{\mathrm{Fib}}
\newcommand{\ASp}{\mathrm{ASp}}
\newcommand{\Sch}{\mathrm{Sch}}
\newcommand{\Mod}{\mathrm{Mod}}
\newcommand{\Set}{\mathrm{Set}}
\newcommand{\CL}{\mathrm{CL}}
\newcommand{\CM}{\mathrm{CM}}
\newcommand{\PSh}{\mathrm{PSh}}
\newcommand{\Sp}{\mathrm{Sp}}
\newcommand{\Alg}{\mathrm{Alg}}
\newcommand{\Ell}{\mathrm{Ell}}
\newcommand{\LT}{\mathrm{LT}}
%\newcommand{\LC}{\mathrm{LC}}
\renewcommand{\L}{\mathrm{L}}
\newcommand{\V}{\mathrm{V}}
\newcommand{\Biring}{\mathrm{Biring}}

%RINGS, FIELDS, MONOIDS
\renewcommand{\O}{\mathcal{O}}
\newcommand{\Q}{\mathbf{Q}}
\newcommand{\Sh}{\mathrm{Sh}}
\newcommand{\Z}{\mathbf{Z}}
\newcommand{\N}{\mathbf{N}}
\newcommand{\F}{\mathbf{F}}
\newcommand{\R}{\mathbf{R}}
\newcommand{\G}{\mathbf{G}}
\newcommand{\C}{\mathbf{C}}
\renewcommand{\k}{\boldsymbol{k}}
\newcommand{\Id}{\mathrm{Id}}

%HOMS
\newcommand{\End}{\mathrm{End}}
\newcommand{\Isom}{\mathrm{Isom}}
\newcommand{\Hom}{\mathrm{Hom}}
\newcommand{\Aut}{\mathrm{Aut}}

%IDEALS
\newcommand{\ideal}[1]{\mathfrak{#1}}
\renewcommand{\a}{\ideal{a}}
\renewcommand{\b}{\ideal{b}}
\renewcommand{\l}{\ideal{l}}
\renewcommand{\d}{\ideal{d}}
\renewcommand{\c}{\ideal{c}}
\newcommand{\m}{\ideal{m}}
\newcommand{\p}{\ideal{p}}
\newcommand{\f}{\ideal{f}}
\newcommand{\g}{\ideal{g}}
\renewcommand{\P}{\ideal{P}}
\newcommand{\D}{\ideal{D}}
\renewcommand{\G}{\ideal{G}}

%SUBSCRIPTS AND SUPERSCRIPTS
\newcommand{\can}{\mathrm{can}}
\newcommand{\univ}{\mathrm{univ}}
\newcommand{\ord}{\mathrm{ord}}
\newcommand{\perf}{\mathrm{perf}}
\newcommand{\proet}{\mathrm{pro\acute{e}t}}
\newcommand{\tors}{\mathrm{tors}}
\newcommand{\ab}{\mathrm{ab}}
\newcommand{\witt}{\mathrm{witt}}
\newcommand{\ec}{\mathrm{ell}}
\newcommand{\sep}{\mathrm{sep}}
\newcommand{\ur}{\mathrm{ur}}
\newcommand{\arch}{\mathrm{arch}}
\newcommand{\dis}{\mathrm{dis}}
\newcommand{\fin}{\mathrm{fin}}
\newcommand{\red}{\mathrm{red}}
\newcommand{\an}{\mathrm{an}}
\newcommand{\ind}{\mathrm{ind}}
\newcommand{\alg}{\mathrm{alg}}
\newcommand{\gh}{\mathrm{gh}}
\newcommand{\str}{\mathrm{str}}
\newcommand{\et}{\textup{\'et}}
\newcommand{\per}{\mathrm{per}}

%SPECIAL MAPS
\newcommand{\id}{\mathrm{id}}
\newcommand{\Fr}{\mathrm{Fr}}
\newcommand{\pr}{\mathrm{pr}}

%SPECIAL SHEAVES
\newcommand{\A}{\mathbf{A}}

%MISCELLANEOUS FUNCTIONS
\newcommand{\height}{\mathrm{ht}}
\newcommand{\rk}{\mathrm{rk}}
\newcommand{\WT}{\mathrm{WT}}

%SPECIAL FUNCTORS
\newcommand{\Inf}{\mathrm{Inf}}
\newcommand{\Spec}{\mathrm{Spec}}
\newcommand{\Div}{\mathrm{Div}}
\renewcommand{\div}{\mathrm{div}}
\newcommand{\Spf}{\mathrm{Spf}}
\newcommand{\Lie}{\mathrm{Lie}}
\newcommand{\Str}{\mathrm{Str}}
\newcommand{\Sym}{\mathrm{Sym}}
\newcommand{\DLog}{\mathrm{DLog}}
\newcommand{\Tan}{\mathrm{Tan}}
\newcommand{\Prin}{\mathrm{P}}
\newcommand{\Ner}{\mathrm{N\acute{e}r}}
\newcommand{\DR}{\mathrm{DR}}
\newcommand{\Eq}{\mathrm{Eq}}
\newcommand{\In}{\mathrm{In}}




